Towards Trace-based Deductive Verification (Tech Report)

Contracts specifying a procedure's behavior in terms of pre- and postconditions are essential for scalable software verification, but cannot express any constraints on the events occurring during execution of the procedure. This necessitates to annotate code with intermediate assertions, preventing full specification abstraction. We propose a logic over symbolic traces able to specify recursive procedures in a modular manner that refers to specified programs only in terms of events. We also provide a deduction system based on symbolic execution and induction that we prove to be sound relative to a trace semantics. Our work generalizes contract-based to trace-based deductive verification.

==> loop-rule-proof.tex <==

Soundness of the $\mathsf{Loop}$ rule requires us to show
$\sigma \models \update\, 
 \judge{\mbox{\lstinline{while}}\,(b)\,s;s'}{\Phi}$
for all states~$\sigma$. 
%
By validity of the first and third premises of the rule,
this reduces to showing
$\sigma \models \judge{\mbox{\lstinline{while}}\,(b)\,s}{\Upsilon(i_0)}$
for all states~$\sigma$. 
%
This can be shown by a course-of-values induction on the value 
of $\mathit{variant}$ in~$\sigma$. 
%
First, observe that the second premise establishes that every time the 
body~$s$ of the loop is executed (which only happens in states where 
$b$~evaluates to true), the value of $\mathit{variant}$ is strictly decreased. 
%
The latter value is an integer which the first premise guarantees to 
be initially non-negative, while the second premise guarantees 
it to stay so, and is thus a natural number. 
%
Now, let $k \geq 0$, and let $\sigma$ be an arbitrary state such that 
the value of $\mathit{variant}$ in~$\sigma$ is~$k$.
%
Assume, as the induction hypothesis, that
$\sigma' \models \judge{\mbox{\lstinline{while}}\,(b)\,s}{\Upsilon(i_0)}$
holds for all states~$\sigma'$ such that the value of $\mathit{variant}$
in~$\sigma'$ is smaller than~$k$.
%
By the local evaluation rules from Figure~\ref{fig:local},
the value of~$b$ in~$\sigma$ is either false, and then the while 
loop terminates immediately, making true the left disjunct of 
the body of the fixed-point formula~$\Upsilon(i_0)$, or else it 
is true and then $s; \mbox{\lstinline{while}}\, (b)\, s$ is executed. 
%
By validity of the second premise of the $\mathsf{Loop}$ 
rule, the loop body~$s$ gives rise to a trace matching~$\Phi_s(i_0)$, 
at the final state of which the value of $\mathit{variant}$ has strictly 
decreased. Thus, the induction hypothesis applies to the continuation
trace produced when executing $\mbox{\lstinline{while}}\, (b)\, s$,
and $X(step^{-1}(i_0))$ is therefore matched by that trace, making
true the right disjunct of the body of~$\Upsilon(i_0)$. 



==> loopRule.tex <==
\subsection{Loops}
\label{sec:loops}

To specify loops one can use finite, unbounded quantification over the
loop body specification, i.e.\ an inductive invariant. Assume that
$\Phi_s(i)$ specifies a given loop body $s$ with parameter $i$.
%
$$
\Upsilon(i)=\mu X(i).\bigl(\stateFml{!b \wedge I(i)}\,\lor\,\stateFml{b \wedge I(i)}\chop\,\Phi_s(i)\chop\,X(step^{-1}(i))\bigr)
$$

The conventional first-order state invariant $I$ would match
$\stateFml{I\land b}\chop\,\Phi_s(i_0)\chop\,\stateFml{I}$.

Let $\Phi_{\mathcal{U}}$ be the specification corresponding to
$\mathcal{U}$.  The loop specification $\Upsilon(i)$ is used inside
the following invariant rule where the overall specification has the
shape $\Phi=\Phi_{\mathcal{U}}\chop\Upsilon(i_0)\chop\,\Phi'$.

\Todo{Add explanation: $\mu$ in $\Upsilon(i)$ enforce termination, therefore we need $variant$}
%
%$$
%\seqRule{Loop_{anotherTry}}{
%\sequent{}{\update\judge{\mbox{\lstinline|skip|}}{\Phi_{\update}\chop\,\stateFml{I(i_0)}\chop\stateFml{i_0\geq 0}}}\\
%\seq{b,\,i_0\geq 0,\,\judge{\mbox{\lstinline{while}}\,(b)\,s}{\Upsilon(step^{-1}(i_0))}}
%{\judge{\mbox{\lstinline{while}}\,(b)\,s}{\Upsilon(i_0)}}\\
%\seq{\judge{\mbox{\lstinline{while}}\,(b)\,s'}{\Upsilon(i_0)}}
%{\judge{\mbox{\lstinline{while}}\,(b)\,s;s'}{\Upsilon(i_0)\chop\Phi'}}
%}{
%\sequent{}{\update\,\judge{\mbox{\lstinline{while}}\,(b)\,s;s'}{\Phi}}
%}
%$$

While \ruleName{TrAbs} rule is applied only after symbol execution terminates,
the sequence of statement following a loop has to be executed after the loop has been removed.
If the loop occurs in a method body, this sequence is always ended by a return statement.
Therefore information about the context from might be lost if not explicitly reintroduced.
For this reason we define the following function that retrieve the $\startEv$ from the sequence of updates
before the loop:
  $$StartEvent(\update) =\begin{cases}
    \startEv(m,e,i)& \text{ if \ } \update=\startEv(m,e,i)\update'\\
    NullEv & \text{otherwise}
  \end{cases}$$\\
where  $\upP{NullEv} = \epsilon$, and $NullEv \chop \tau = \tau$.
Since there can be only one $\startEv$ in a sequence of updates and it is the first element of the sequence
the retrieval is quite straightforward.
If before the loop no $\startEv$ has been generated then it means that the loop is in the main block, 
and we do not need to retrieve the context because no return statement can occur.

$$
\seqRule{Loop}{
\sequent{}{\upl\startEv(m,e,i)\upr\update\judge{}{\Phi_{\update}\chop\,\stateFml{I(i_0)\wedge variant\geq 0}}}\\
\seq{b,I(i_0),oldVar\doteq variant}{\judge{s}}{\Phi_{s}(i_0)\chop\stateFml{I(i_0) \wedge variant\geq 0 \wedge oldVar>variant}}\\
%\seq{b,I(i_0),\judge{\mbox{s}}{\Upsilon(i_0)}}{\judge{s; \mbox{\lstinline|if|}~(b)~s}}{\Upsilon(step(i_0))}\\
\seq{!b,\,I(i_0)}{\judge{\mbox{$\upP{\startEv(m,e,i)} s'$}}{\startEv(m,e,i) \chop \ \Phi'}}\\
}{
\sequent{}{\upl\startEv(m,e,i)\upr\mathcal{U}\,\judge{\mbox{\lstinline{while}}\,(b)\,s;s'}{\Phi}}
}
$$




%$$
%\seqRule{Loop_{new}}{
%\sequent{}{\update\judge{\mbox{\lstinline|skip|}}{\Phi_{\update}\chop\,\stateFml{I(i_0)}}}\\
%\seq{b,I(i_0),\judge{\mbox{s}}{\Upsilon(i_0)}}{\judge{s; \mbox{\lstinline|if|}~(b)~s}}{\Upsilon(step(i_0))}\\
%\seq{\judge{\mbox{\lstinline{while}}(b) s}{\Upsilon(i_0)}}{\judge{\mbox{\lstinline{while}}(b)s;s'}{\Upsilon(i_0)\chop\,\Phi'}}\\
%}{
%\sequent{}{\mathcal{U}\,\judge{\mbox{\lstinline{while}}\,(b)\,s;s'}{\Phi}}
%}
%$$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mycomment{%%%%%
\Todo{%%%
To prove soundness of the rule, we shall prove 
$\sigma \models \update\, 
 \judge{\mbox{\lstinline{while}}\,(b)\,s;s'}{\Phi}$
for all~$\sigma$
by mathematical induction on the number~$\xi (\sigma)$ 
of executions of the loop body~$s$ when executing 
$\mbox{\lstinline{while}}\,(b)\,s$ from the state
$\mathit{last} (\eval{\update}{\singleton{\sigma}})$.

~~In the base case of $\xi (\sigma) = 0$, since the loop 
body is never executed, we must have
$\sigma \models \update (!b)$.
Then, by the local evaluation rules (Figure~\ref{fig:local}), 
the definition of the global semantics with updates, 
and Proposition~\ref{prop:glob-sem-comp-update},
$   \eval{\update\,\mbox{\lstinline{while}}\,(b)\,s;s'}{\singleton{\sigma}}
  = \eval{\update}{\singleton{\sigma}}  
    \,\chopSem\,
    \eval{\mbox{\lstinline{while}}\,(b)\,s;s'}{\tau}
  = \eval{\update}{\singleton{\sigma}}  
    \,\chopSem\,
    \eval{s'}{\tau}
  = \eval{\update\, s'}{\singleton{\sigma}} $
must hold, where 
$\tau = \eval{\update}{\singleton{\sigma}}$.
By the assumed validity of the first premise, also 
$\sigma \models \update \judge{s'}{\Phi}$ must hold, 
and hence
$ \sigma \models \update\,
  \judge{\mbox{\lstinline{while}}\,(b)\,s;s'}{\Phi} $.

~~For the induction case [flawed!], assume (as the induction 
hypothesis) that we have
$ \sigma \models \update\,
  \judge{\mbox{\lstinline{while}}\,(b)\,s;s'}{\Phi} $
for all~$\sigma$ such that $\xi (\sigma) = k$.
Let~$\sigma'$ be any state such that  $\xi (\sigma') = k+1$.
Then, since the loop body is executed at least once, 
$\sigma' \models \update (b)$ must hold, and therefore also
%
$ \eval{\update\,\mbox{\lstinline{while}}\,(b)\,s;s'}
       {\singleton{\sigma'}}
  \stackrel {\mbox{\tiny (1)}}{=} 
  \eval{\update\,s;\mbox{\lstinline{while}}\,(b)\,s;s'}
       {\singleton{\sigma'}}
  \stackrel {\mbox{\tiny (2)}}{=} 
  \eval{\update\,s}{\singleton{\sigma'}}
  \,\chopSem\,
  \eval{\mbox{\lstinline{while}}\,(b)\,s;s'}{\tau} $
by Proposition~\ref{prop:glob-sem-comp-update}, where
$\tau = \eval{\update\,s}{\singleton{\sigma'}}$. 
%
Now, $\xi (\mathit{last}(\tau)) = k$, and then, by the 
induction hypothesis applied to state $\mathit{last}(\tau)$,
we have 
$ \mathit{last}(\tau) \models \update\,
  \judge{\mbox{\lstinline{while}}\,(b)\,s;s'}{\Phi} $.
Hence, by the shape of~$\Phi$ and by \ldots,
$ \mathit{last}(\tau) \models 
  \judge{\mbox{\lstinline{while}}\,(b)\,s;s'}
        {\Upsilon(i_0)\chop\,\Phi'} $.
From this, equation~(2) above, and the assumed validity
of the second premise, we can infer that
$ \sigma' \models 
  \judge{s;\mbox{\lstinline{while}}\,(b)\,s;s'}
        {\Upsilon(i_0)\chop\,\Phi'} $,
which entails
$ \sigma' \models \update\,
  \judge{s;\mbox{\lstinline{while}}\,(b)\,s;s'}{\Phi} $.
Therefore, by equation~(1) above, we finally obtain
$ \sigma' \models \update\,
  \judge{\mbox{\lstinline{while}}\,(b)\,s;s'}{\Phi} $.

This concludes the proof. \qed
}

\noindent
Dilian: The starting point could be the following ``basic'' 
rule for loops:
%
$$
\seqRule{BasicLoop}{
\sequent{!b}{\judge{\mbox{\sf skip}}{\Phi_I}}~~~~~ %\\
\seq{\Gamma, b,\,\judge{\mbox{\lstinline{while}}\,(b)\,s}{\Phi_I}}{\judge{s;\mbox{\lstinline{while}}\,(b)\,s}{\Phi_I}}
}{
\sequent{}{\judge{\mbox{\lstinline{while}}\,(b)\,s}{\Phi_I}}
}
$$
%
where~$\Phi_I$ is a loop invariant.
}%%%%% end comment


==> misc.tex <==

\subsubsection{Improve Readability}
\label{sec:usability}

Introduce syntactic sugar in the form of specification patterns. For
example, expression~\eqref{eq:muEx} might be written as follows:

\begin{align*}
  \mathbf{letrec}\,C_m(n).\ \bigl(\ & n\doteq 0 \Rightarrow m(0)\finiteNoM{m}return(0);\\
  & n>1 \Rightarrow m(n)\finiteNoM{m}C_m(n-1)\finiteNoM{m}return(n)\ \bigr)
\end{align*}

The call identifiers and names of return variables can be inferred, so
expression~\eqref{eq:muEx} can be automatically generated from such a pattern.

\emph{Do something similar for loop invariants}

\emph{I suggest a notation similar to $\cdot\cdot$ that stands for all
  traces of \emph{straight line code} (i.e.\ no loops, no calls). This
  will help in writing specifications of programs with loops. One idea
  is to use the notation ``---''.}

\lstset{language=[JML]Java,mathescape=true}

\begin{lstlisting}
public interface I {
  /*@ public trace_contract
    @   letrec $C_m(n)\,\ldots$ ; 
    @   conforms_to $C_m$;
    @*/
  public int m(int k);
}
\end{lstlisting}




==> prooftree.tex <==

\newpage
\section{Examples [To be distributed to previous sections]}

\begin{lstlisting}[escapechar=\%]
  int m(int k) {
    r;
    if (k!=0) 
      { r = m(k-1);r+1 };
    return r;
  }
\end{lstlisting}
\begin{align}
  \mu X_m(n,i).&\stateFml{n\doteq 0}\chop\startEv(m,0,i)\finiteNoM{m}\finishEv(m,0,i)\concat\stateFml{res_i\doteq 0} \label{eq:muEx1}\\
               & \vee\stateFml{n>0}\chop\startEv(m,n,i)\finiteNoM{m}X_m(n-1,\#(i))\finiteNoM{m}\finishEv(m,n,i)\concat\stateFml{res_i\doteq n}\notag
\end{align}



\begin{align*}
\mathbf{C}_m=\forall
n,i.(n\geq0\rightarrow\judge{m(n)}{X_m(n,i)}\chop \stateFml{res_i\doteq n})\\
\end{align*}
$b_m$ = {r; s}

\noindent s:=\textbf{if}$(k!=0)$\{$r=m(k-1); r=r+1;$\} \textbf{return}~r

\newpage
%\newgeometry{left=0.1cm,right=0.1cm,bottom=0.1cm}
\noindent The rules highlighted in \Blue{blue} are the ones introduced in this paper, the one highlighted in \Red{red} are not defined.\\
Highlighting pointing out the targets of each rule application are provided in \Red{red} (for \Red{targets dropped} by rule), and \Blue{blue} (for \Blue{targets not dropped} by rule).

\scalebox{0.75}{
\begin{minipage}{\textwidth}
\begin{prooftree}
  \AxiomC{(a)\quad\quad\quad\quad\quad}
  \AxiomC{(b)}
  \BinaryInfC{\RuleL{\Blue{Cond}}$\seq {n'\geq0,\,\mathbf{C}_m}{\judge{\underbrace{\upP{\startEv(m,n',0)}\upP{k':=n'}\upP{r':=0}}_{\mathcal{U}} \Blue{s}[k/k',r/r']}{X_m(n',0)}}$}
  \UnaryInfC{\RuleL{\Blue{VarDecl}}$\seq{n'\geq0,\,\mathbf{C}_m}{\judge{\upP{\startEv(m,n',0)}\upP{k':=n'} \{\Blue{r};s[k/k']\}}{X_m(n',0)}}$}
  \UnaryInfC{\RuleL{\Blue{Assign}}$\seq{n'\geq0,\,\mathbf{C}_m}{\judge{\upP{\startEv(m,n',0)} \Blue{k'=n'};\{r;s[k/k']\}}{X_m(n',0)}}$}
  \UnaryInfC{$\seq{n'\geq0,\,\mathbf{C}_m}{\judge{inline(m,n')}{X_m(n',0)}}$}
  \UnaryInfC{\RuleL{\Blue{ProcedureContract}}$\seq{}{\Blue{\mathbf{C}_m}}$}
\end{prooftree}
With $\update=\upP{\startEv(m,n',0)}\upP{k':=n'}\upP{r':=0}$\\

Continue with (a):
\begin{prooftree}
  \AxiomC{$\seq{n'\doteq0}{n'\doteq0}$}
  \AxiomC{$\seq{}{\judge{\upP{res_0:=0}}{\stateFml{res_0 \doteq 0}}}$}
  \UnaryInfC{\RuleL{\Red{PrefixEv}}$\seq{}{\judge{\Red{\upP{\finishEv(m,0,0)}}\upP{res_0:=0}}{\Red{\finishEv(m,0,0)}\concat\stateFml{res_0\doteq 0}}}$}
  \UnaryInfC{\RuleL{\Red{FiniteTraceEmptyPrefix}}$\seq{}{\judge{\Blue{\upP{\finishEv(m,0,0)}}\upP{res_0:=0}}{\Red{\finiteNoM{m}}\finishEv(m,0,0)\concat\stateFml{res_0\doteq 0}}}$}
  \UnaryInfC{\RuleL{\Red{PrefixEv}}$\seq{}{\judge{\Red{\upP{\startEv(m,0,0)}}\upP{\finishEv(m,0,0)}\upP{res_0:=0}}{\Red{\startEv(m,0,0)}\finiteNoM{m}\finishEv(m,0,0)\concat\stateFml{res_0\doteq 0}}}$}
  \BinaryInfC{\RuleL{\Blue{Prestate}}$\seq{\Blue{n'\doteq0}}{\judge{\upP{\startEv(m,0,0)}\upP{\finishEv(m,0,0)}\upP{res_0:=0}}{\stateFml{\Blue{n'\doteq 0}}\chop\startEv(m,0,0)\finiteNoM{m}\finishEv(m,0,0)\concat\stateFml{res_0\doteq 0}}}$}
  \UnaryInfC{\RuleL{dropUpdate \, x2}$\seq{n'\doteq0}{\judge{\upP{\startEv(m,0,0)}\Red{\upP{k':=0}\upP{r':=0}}\upP{\finishEv(m,0,0)}\upP{res_0:=0}}{X_m(0,0)}}$}
  \UnaryInfC{\RuleL{applyUpdate}$\seq{n'\doteq0}{\judge{\upP{\startEv(m,0,0)}\upP{k':=0}\upP{\Blue{r':=0}}\upP{\finishEv(m,\Blue{r'},0)}\upP{res_0:=\Blue{r'}}}{X_m(0,0)}}$}
  \UnaryInfC{\RuleL{applyEqRigid}$\seq{\Blue{n'\doteq0}}{\judge{\upP{\startEv(m,\Blue{n'},0)}\upP{k':=\Blue{n'}}\upP{r':=0}\upP{\finishEv(m,r',0)}\upP{res_0:=r'}}{X_m(\Blue{n'},0)}}$}
  \UnaryInfC{\RuleL{\Blue{Assign}}$\seq{n'\doteq0}{\judge{\mathcal{U}\upP{\finishEv(m,r',0)}\Blue{res_0=r'}}{X_m(n',0)}}$}
  \UnaryInfC{\RuleL{\Blue{Return}}$\seq{n'\geq0,\,\mathbf{C}_m,\,\mathcal{U}(k'=0)}{\judge{\mathcal{U} \,\Blue{\returnStmt{r'}}}{X_m(n',0)}}$}
  \UnaryInfC{(a)}
\end{prooftree}

Continue with (b):
\begin{prooftree}
  \AxiomC{$\seq{n'>0}{n'\geq 0}$} 
  \UnaryInfC{\RuleL{dropUpdate}$\seq{n'>0}{\Red{\update_1}(n'\geq 0)}$} 
  \AxiomC{$\seq{n'>0}{n'>0}$} 
  \AxiomC{$\seq{}{\judge{\upP{\startEv(m,n',0)}}{\startEv(m,n',0)}}$} 
  \BinaryInfC{\RuleL{\Blue{Prestate}}$\seq{\Blue{n'>0}}{\judge{\upP{\startEv(m,n',0)}}{\Blue{\stateFml{n'>0}}\chop \startEv(m,n',0)}}$} 
  \UnaryInfC{\RuleL{\Red{FiniteTraceEmptyPostfix}}$\seq{n'>0}{\judge{\Blue{\upP{\startEv(m,n',0)}}}{\stateFml{n'>0}\chop \startEv(m,n',0)\Red{\finiteNoM{m}}}}$} 
  \AxiomC{\quad (c)} 
  \TrinaryInfC{\RuleL{\Blue{TraceAbs}}$\seq{n'>0, \mathbf{C}_m}{\judge{\upP{\underbrace{\startEv(m,n',0)}_{\Blue{\update_1}}} \Blue{\upP{r':=m(n'-1)}}\underbrace{\upP{r':=r'+1}\upP{\finishEv(m,r',0)}\upP{res_0:=r'}}_{\Blue{\update_2}}  }{X_m(n',0)}}$}
  \UnaryInfC{\RuleL{\Blue{Return}}$\seq{n'>0, \mathbf{C}_m}{\judge{\upP{\startEv(m,n',0)} \upP{r':=m(n'-1)}\upP{r':=r'+1}\,\Blue{\returnStmt{r'}} }{X_m(n',0)}}$}
  \UnaryInfC{\RuleL{dropUpdate \, x2}$\seq{n'>0, \mathbf{C}_m}{\judge{\upP{\startEv(m,n',0)}\Red{\upP{k':=n'}\upP{r':=0}} \upP{r':=m(n'-1)}\upP{r':=r'+1}\,\returnStmt{r'} }{X_m(n',0)}}$}
  \UnaryInfC{\RuleL{applyUpdate}$\seq{n'>0, \mathbf{C}_m}{\judge{\upP{\startEv(m,n',0)}\Blue{\upP{k':=n'}}\upP{r':=0} \upP{r':=m(\Blue{k'}-1)}\upP{r':=r'+1}\,\returnStmt{r'} }{X_m(n',0)}}$}
  \UnaryInfC{\RuleL{\Blue{Assign} \, x2}$\seq{n'>0, \mathbf{C}_m}{\judge{\upP{\startEv(m,n',0)}\upP{k':=n'}\upP{r':=0} \, \Blue{r':=m(k'-1)};\Blue{r':=r'+1};\returnStmt{r'} }{X_m(n',0)}}$}
  \UnaryInfC{(b)}
\end{prooftree}
% U_2 = \upP{r':=r'+1}\upP{\finishEv(m,r',0)}\upP{res_0:=r'}
\ \ \ \ With $n>0$ we have:
$X_m(n',0)=\stateFml{n>0}\chop\underbrace{\startEv(m,n',0)\finiteNoM{m}}_{X_1}X_m(n'-1,k)\underbrace{\finiteNoM{m}\finishEv(m,n',0)\concat\stateFml{res_i\doteq n'}}_{X_2}, \text{ where $k$ is fresh}$

Continue with (c):
\begin{prooftree}
  \AxiomC{\LeftLabel{}$\seq{}{\judge{\upP{res_0:=n'}}{\stateFml{res_0\doteq n'}}}$} 
  \UnaryInfC{\RuleL{\Red{PrefixEv}}$\seq{}{\judge{\Red{\upP{\finishEv(m,n',0)}}\upP{res_0:=n'}}{\Red{\finishEv(m,n',0)}\concat\stateFml{res_0\doteq n'}}}$} 
  \UnaryInfC{\RuleL{\Red{FiniteTraceEmptyPrefix}}$\seq{}{\judge{\Blue{\upP{\finishEv(m,n',0)}}\upP{res_0:=n'}}{\Red{\finiteNoM{m}}\finishEv(m,n',0)\concat\stateFml{res_0\doteq n'}}}$} 
  \UnaryInfC{\RuleL{apply+dropUpdate}$\seq{}{\judge{\Blue{\upP{r':=n'}}\upP{\finishEv(m,\Blue{r'},0)}\upP{res_0:=\Blue{r'}}}{\finiteNoM{m}\finishEv(m,n',0)\concat\stateFml{res_0\doteq n'}}}$} 
  \UnaryInfC{\RuleL{apply+dropUpdate}$\seq{}{\judge{\Blue{\upP{r':=n'-1}}\upP{r':=\Blue{r'}+1}\upP{\finishEv(m,r',0)}\upP{res_0:=r'}}{\finiteNoM{m}\finishEv(m,n',0)\concat\stateFml{res_0\doteq n'}}}$} 
  \UnaryInfC{\RuleL{applyEq+dropEq}$\seq{\Blue{res_k \doteq n'-1}}{\judge{\upP{r':=\Blue{res_k}}\upP{r':=r'+1}\upP{\finishEv(m,r',0)}\upP{res_0:=r'}}{\finiteNoM{m}\finishEv(m,n',0)\concat\stateFml{res_0\doteq n'}}}$} 
  \UnaryInfC{(c)} 
\end{prooftree}
\end{minipage}
}

%\restoregeometry

\subsection{Missing Rules: suggestions}

$$
\seqRule{PrefixEv}{
\sequent{}{\update \judge{s}{\Phi}}
}{
\sequent{}{\judge{\upP{\ev{m,e}} \, \update s}{{\ev{m,e}\chop \, \Phi}}}
}
$$

$$
\seqRule{FiniteTraceEmptyPrefix}{
\sequent{}{\upP{\ev{m,e}} \, \update \judge{s}{\Phi}}
}{
\sequent{}{\judge{\upP{\ev{m,e}} \, \update s}{\finiteNoM{m}\chop \, \Phi}}
}
$$

$$
\seqRule{FiniteTraceEmptyPostfix}{
\sequent{}{\update \upP{\ev{m,e}} \judge{}{\Phi}}
}{
\sequent{}{\judge{\update \upP{\ev{m,e}}}{\Phi\chop\finiteNoM{m} }}
}
$$

$$
\seqRule{Composition}{
\sequent{}{\update \judge{}{\Phi_1}\qquad \update' s \judge{}{\Phi_2}}
}{
\sequent{}{\judge{\update \update' s}{\Phi_1\chop\Phi_2 }}
}
$$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> tikzlibrarytikzmark.code.tex <==
%%
%% This is file `tikzlibrarytikzmark.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `tikzlibrary')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\ProvidesFile{tikzlibrarytikzmark.code.tex}[%
  2021/02/16
  v1.10
  TikZ library for marking positions in a document]
\RequirePackage{expl3, l3keys2e, xparse}
\tikzset{%
  remember picture with id/.style={%
    remember picture,
    overlay,
    save picture id=#1,
  },
  every picture/.append style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage%
      \edef\pgf@temp{%
        \noexpand\write\noexpand\pgfutil@auxout{%
          \string\savepicturepage%
          {\pgfpictureid}{\noexpand\arabic{page}}%
        }%
      }%
      \pgf@temp
      \fi%
    },
  },
  check picture id/.code={
    \ifpgfrememberpicturepositiononpage
    \@ifundefined{pgf@sys@pdf@mark@pos@\pgfpictureid}{%
      \tikzset{%
        name prefix/.get=\tzmk@name@prefix,
        name prefix/.prefix=discard-,
        execute at end picture={%
          \tikzset{name prefix/.expand once=\tzmk@name@prefix}%
        },
      }%
    }{}%
    \fi
  },
  maybe define node/.style={%
    execute at end picture={%
      \ifpgfrememberpicturepositiononpage
      \@ifundefined{pgf@sh@pi@\tikz@pp@name{#1}}{%
        \pgfnodealias{\tikz@pp@name{#1}}{discard-\tikz@pp@name{#1}}%
      }{}%
      \fi
    }%
  },
  save picture id/.code={%
      \protected@write\pgfutil@auxout{}{%
      \string\savepointas%
      {\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
  },
  if picture id/.code args={#1#2#3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{
      \pgfkeysalso{#2}%
    }
  },
  next page/.is choice,
  next page vector/.initial={\pgfqpoint{0pt}{0pt}},
  next page/below/.style={%
    next page vector={\pgfqpoint{0pt}{-\the\paperheight}}%
  },
  next page/above/.style={%
    next page vector={\pgfqpoint{0pt}{\the\paperheight}}%
  },
  next page/left/.style={%
    next page vector={\pgfqpoint{-\the\paperwidth}{0pt}}%
  },
  next page/right/.style={%
    next page vector={\pgfqpoint{\the\paperwidth}{0pt}}%
  },
  next page/ignore/.style={%
    next page vector={\pgfqpoint{0pt}{0pt}}%
  },
  if tikzmark on current page/.code n args={3}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#3}%
    }{%
      \@ifundefined{%
        save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname
      }{%
        \pgfkeysalso{#3}%
      }{%
        \ifnum\csname save@pg@%
        \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
        \endcsname=\the\value{page}\relax%
        \pgfkeysalso{#2}%
        \else
        \pgfkeysalso{#3}%
        \fi
      }%
    }%
  },
  if tikzmark on page/.code n args={4}{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      \pgfkeysalso{#4}%
    }{%
      \@ifundefined{%
        save@pg@\csname save@pt@\tikzmark@pp@name{#1}@label\endcsname%
      }{%
        \pgfkeysalso{#4}%
      }{%
        \ifnum\csname save@pg@%
        \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
        \endcsname=#2\relax%
        \pgfkeysalso{#3}%
        \else
        \pgfkeysalso{#4}%
        \fi
      }%
    }%
  },
  tikzmark prefix/.initial=,%
  tikzmark suffix/.initial=,%
}
\def\tikzmark@pp@name#1{%
  \csname pgfk@/tikz/tikzmark prefix\endcsname%
  #1%
  \csname pgfk@/tikz/tikzmark suffix\endcsname%
}%
\def\savepointas#1#2#3#4{%
  \expandafter\gdef\csname save@pt@#1\endcsname{#2}%
  \expandafter\gdef\csname save@pt@#1@offset\endcsname%
  {\pgfqpoint{#3}{#4}}%
}
\def\savepicturepage#1#2{%
  \expandafter\gdef\csname save@pg@#1\endcsname{#2}%
}
\def\tikzmarkalias#1#2{%
  \pgf@node@gnamelet{save@pt@#1}{save@pt@#2}%
  \pgf@node@gnamelet{save@pt@#1@offset}{save@pt@#2@offset}%
}
\def\tmk@labeldef#1,#2\@nil{%
  \edef\tmk@label{\tikzmark@pp@name{#1}}%
  \def\tmk@def{#2}%
}
\tikzdeclarecoordinatesystem{pic}{%
  \pgfutil@in@,{#1}%
  \ifpgfutil@in@%
    \tmk@labeldef#1\@nil
  \else
    \tmk@labeldef#1,(0pt,0pt)\@nil
  \fi
  \@ifundefined{save@pt@\tmk@label}{%
    \tikz@scan@one@point\pgfutil@firstofone\tmk@def
  }{%
    \pgfsys@getposition{\csname save@pt@\tmk@label\endcsname}%
    \save@orig@pic%
    \pgfsys@getposition{\pgfpictureid}\save@this@pic%
    \pgf@process{\pgfpointorigin\save@this@pic}%
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process{\pgfpointorigin\save@orig@pic}%
    \advance\pgf@x by -\pgf@xa
    \advance\pgf@y by -\pgf@ya
    \pgf@xa=\pgf@x
    \pgf@ya=\pgf@y
    \pgf@process%
    {\pgfpointorigin\csname save@pt@\tmk@label @offset\endcsname}%
    \advance\pgf@xa by \pgf@x
    \advance\pgf@ya by \pgf@y
      \@ifundefined{save@pg@\csname save@pt@\tmk@label\endcsname}{}{%
        \@ifundefined{save@pg@\pgfpictureid}{}{%
          \pgfkeysvalueof{/tikz/next page vector}%
        \edef\tmk@pg{%
          \the\numexpr \csname save@pg@%
          \csname save@pt@\tmk@label\endcsname\endcsname%
          -
          \csname save@pg@\pgfpictureid\endcsname\relax%
        }%
        \ifnum \tmk@pg > 0 \relax
        \advance \pgf@xa by \pgf@x\relax
        \advance \pgf@ya by \pgf@y\relax
        \fi
        \ifnum \tmk@pg < 0 \relax
        \advance \pgf@xa by -\pgf@x\relax
        \advance \pgf@ya by -\pgf@y\relax
        \fi
        }%
      }%
      \pgf@x=\pgf@xa
      \pgf@y=\pgf@ya
    \pgftransforminvert
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
  }%
}
\newcommand\tikzmark@outside[2][]{%
\tikzset{external/export next/.try=false}%
\tikz[remember picture with id=#2]{#1}%
}
\def\tikzmark@inside#1#2{%
  \tikzset{remember picture}%
  \tikz@scan@one@point\pgfutil@firstofone#2\relax
  \protected@write\pgfutil@auxout{}{%
    \string\savepointas%
    {\tikzmark@pp@name{#1}}{\pgfpictureid}{\the\pgf@x}{\the\pgf@y}}%
}
\def\tikzmark{%
  \ifx\pgfpictureid\@undefined
  \let\tikzmark@next=\tikzmark@outside
  \else
  \relax
  \ifx\scope\tikz@origscope\relax
  \let\tikzmark@next=\tikzmark@outside
  \else
  \let\tikzmark@next=\tikzmark@inside
  \fi
  \fi
  \tikzmark@next%
}
\newcommand\pgfmark[1]{%
    \bgroup
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
      \pgfsys@markposition{\pgfpictureid}%
    \edef\pgf@temp{%
      \noexpand\write\noexpand\pgfutil@auxout{%
        \string\savepicturepage{\pgfpictureid}{\noexpand\arabic{page}}}}%
    \pgf@temp
    \protected@write\pgfutil@auxout{}{%
      \string\savepointas{\tikzmark@pp@name{#1}}{\pgfpictureid}{0pt}{0pt}}%
    \egroup
  }
\@ifclassloaded{beamer}{
  \renewcommand<>{\tikzmark@outside}[2][]{%
    \only#3{\beameroriginal{\tikzmark@outside}[{#1}]{#2}}%
  }
  \renewcommand<>{\tikzmark@inside}[2]{%
    \only#3{\beameroriginal{\tikzmark@inside}{#1}{#2}}%
  }
}{}
\@ifclassloaded{beamer}{
  \renewcommand<>{\pgfmark}[1]{\only#2{\beameroriginal{\pgfmark}{#1}}}
}{}
\@ifclassloaded{beamer}{
  \tikzset{
    tikzmark suffix=-\the\beamer@slideinframe
  }
}{}
\newif\iftikzmark@
\newcommand\iftikzmark[3]{%
    \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
      #3%
    }{%
      #2%
    }%
}%
\newcommand\iftikzmarkexists[1]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false%
  }{%
    \tikzmark@true%
  }%
  \iftikzmark@
}%
\newcommand\iftikzmarkonpage[2]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false
  }{%
    \@ifundefined{save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname}{%
      \tikzmark@false
    }{%
      \ifnum\csname save@pg@%
      \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
      \endcsname=#2\relax%
      \tikzmark@true
      \else
      \tikzmark@false
      \fi
    }%
  }%
  \iftikzmark@
}
\newcommand\iftikzmarkoncurrentpage[1]{%
  \@ifundefined{save@pt@\tikzmark@pp@name{#1}}{%
    \tikzmark@false
  }{%
    \@ifundefined{save@pg@\csname save@pt@\tikzmark@pp@name{#1}\endcsname}{%
      \tikzmark@false
    }{%
      \ifnum\csname save@pg@%
      \csname save@pt@\tikzmark@pp@name{#1}\endcsname%
      \endcsname=\the\value{page}\relax%
      \tikzmark@true
      \else
      \tikzmark@false
      \fi
    }%
  }%
  \iftikzmark@
}
\def\subnode@#1#2#3{%
  \begingroup
  \pgfmark{#2}%
  \setbox\pgfnodeparttextbox=\hbox\bgroup #3\egroup
  \def\tikz@fig@name{#2}%
  \tikzset{every subnode/.try,#1}%
  \pgfpointorigin
  \tikz@scan@one@point\pgfutil@firstofone(pic cs:#2)\relax
  \advance\pgf@x by .5\wd\pgfnodeparttextbox
  \advance\pgf@y by .5\ht\pgfnodeparttextbox
  \advance\pgf@y by -.5\dp\pgfnodeparttextbox
  \pgftransformshift{}%
  \setbox\@tempboxa=\hbox\bgroup
  {%
    \let\pgf@sh@savedmacros=\pgfutil@empty% MW
    \let\pgf@sh@savedpoints=\pgfutil@empty%
    \def\pgf@sm@shape@name{rectangle}% CJ % TT added prefix!
    \pgf@sh@s@rectangle%
    \pgf@sh@savedpoints%
    \pgf@sh@savedmacros% MW
    \pgftransformshift{%
      \pgf@sh@reanchor{rectangle}{center}%
      \pgf@x=-\pgf@x%
      \pgf@y=-\pgf@y%
    }%
    \expandafter\pgfsavepgf@process\csname pgf@sh@sa@\tikz@fig@name\endcsname{%
      \pgf@sh@reanchor{rectangle}{center}% FIXME : this is double work!
    }%
    % Save the saved points and the transformation matrix
    \edef\pgf@node@name{\tikz@fig@name}%
    \ifx\pgf@node@name\pgfutil@empty%
    \else%
    \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{rectangle}%
    \edef\pgf@sh@@temp{%
      \noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
    \expandafter\pgf@sh@@temp\expandafter{%
      \pgf@sh@savedpoints}%
    \edef\pgf@sh@@temp{%
      \noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
    \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
    \pgfgettransform\pgf@temp
    \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
    \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
    \fi%
  }%
  \egroup
  \box\pgfnodeparttextbox
  \endgroup
}

\newcommand\subnode[3][]{%
  \ifmmode
  \mathchoice{%
    \subnode@{#1}{#2-d}{\(\displaystyle #3\)}%
  }{%
    \subnode@{#1}{#2-t}{\(\textstyle #3\)}%
  }{%
    \subnode@{#1}{#2-s}{\(\scriptstyle #3\)}%
  }{%
    \subnode@{#1}{#2-ss}{\(\scriptscriptstyle #3\)}%
  }%
  \let\pgf@nodecallback\pgfutil@gobble
  \def\tzmk@prfx{pgf@sys@pdf@mark@pos@pgfid}%
  \edef\tzmk@pic{\tzmk@prfx\the\pgf@picture@serial@count}
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-1\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-2\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-3\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \pgfutil@ifundefined{pgf@sh@ns@#2}{%
    \pgfnodealias{#2}{#2-t}%
    \tikzmarkalias{#2}{#2-t}%
  }{}%
  \else
    \pgfnodealias{#2}{#2-d}%
    \tikzmarkalias{#2}{#2-d}%
  \fi
  \else
    \pgfnodealias{#2}{#2-t}%
    \tikzmarkalias{#2}{#2-t}%
  \fi
  \else
    \pgfnodealias{#2}{#2-s}%
    \tikzmarkalias{#2}{#2-s}%
  \fi
  \else
    \pgfnodealias{#2}{#2-ss}%
    \tikzmarkalias{#2}{#2-ss}%
  \fi
  \else
    \subnode@{#1}{#2}{#3}%
  \fi
}

\def\tikzmarknode@#1#2#3{%
\tikzset{external/export next/.try=false}%
  \tikz[%
    remember picture,
    save picture id={#2},
    check picture id,
    maybe define node={#2},
    baseline=(#2.base),
    every tikzmarknode picture/.try
  ] {
    \node[
      anchor=base,
      inner sep=0pt,
      minimum width=0pt,
      name={#2},
      node contents={#3},
      every tikzmarknode/.try,
      #1
  ]}%
}

\newcommand\tikzmarknode[3][]{%
  \ifmmode
  \mathchoice{%
    \tikzmarknode@{#1}{#2-d}{\(\displaystyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-t}{\(\textstyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-s}{\(\scriptstyle #3\)}%
  }{%
    \tikzmarknode@{#1}{#2-ss}{\(\scriptscriptstyle #3\)}%
  }%
  \let\pgf@nodecallback\pgfutil@gobble
  \def\tzmk@prfx{pgf@sys@pdf@mark@pos@pgfid}%
  \edef\tzmk@pic{\tzmk@prfx\the\pgf@picture@serial@count}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-1\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-2\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
\edef\tzmk@pic{\tzmk@prfx\the\numexpr\the\pgf@picture@serial@count-3\relax}%
  \expandafter\ifx\csname\tzmk@pic\endcsname\relax
  \pgfutil@ifundefined{pgf@sh@ns@\tikz@pp@name{#2}}{%
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-t}}%
    \tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-t}}%
  }{}%
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-d}}%
    \tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-d}}%
  \fi
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-t}}%
    \tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-t}}%
  \fi
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-s}}%
    \tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-s}}%
  \fi
  \else
    \pgfnodealias{\tikz@pp@name{#2}}{\tikz@pp@name{#2-ss}}%
    \tikzmarkalias{\tikzmark@pp@name{#2}}{\tikzmark@pp@name{#2-ss}}%
  \fi
  \else
    \tikzmarknode@{#1}{#2}{#3}%
  \fi
}
\def\usetikzmarklibrary{%
  \pgfutil@ifnextchar[{\use@tikzmarklibrary}{\use@@tikzmarklibrary}%
  }%}
\def\use@tikzmarklibrary[#1]{\use@@tikzmarklibrary{#1}}
\def\use@@tikzmarklibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikzmark@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let%
      \csname tikzmark@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikzmark@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikzmark@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \pgfutil@InputIfFileExists{tikzmarklibrary\pgf@temp.code.tex}{}{
          \PackageError{tikzmark}{I did not find the tikzmark extras library '\pgf@temp'.}{}
        }%
      \catcode`\@=\csname tikzmark@library@#1@atcode\endcsname
      \catcode`\|=\csname tikzmark@library@#1@barcode\endcsname
      \fi%
    \fi
  }%
}

\ExplSyntaxOn
\prop_new:N \g__sn_prop
\tl_new:N \l__sn_tmpa_tl
\tl_new:N \l__sn_tmpb_tl
\tl_new:N \l__open_bracket_tl
\tl_set:Nn  \l__open_bracket_tl {[} %]
\tl_new:N \l__sn_group_tl
\clist_new:N \l__sn_nodes_clist
\bool_new:N \l__sn_file_bool
\bool_new:N \g__sn_preamble_bool
\bool_set_true:N \g__sn_preamble_bool
\msg_new:nnn {tikzmark} {no file} {File~ "#1"~ doesn't~ exist.}
\msg_new:nnn {tikzmark} {loading nodes} {Loading~ nodes~ from~ "#1".}
\dim_new:N \l__sn_x_dim
\dim_new:N \l__sn_y_dim
\dim_new:N \l__sn_xa_dim
\dim_new:N \l__sn_ya_dim
\tl_new:N \l__sn_centre_tl

\tl_new:N \l__sn_transformation_tl
\tl_set:Nn \l__sn_transformation_tl {{1}{0}{0}{1}{0pt}{0pt}}
\iow_new:N \g__sn_stream
\bool_new:N \g__sn_stream_bool
\tl_new:N \g__sn_filename_tl
\tl_gset:Nx \g__sn_filename_tl {\c_sys_jobname_str}

\cs_new_nopar:Npn \sn_open_stream:
{
  \bool_if:NF \g__sn_stream_bool
  {
    \iow_open:Nn \g__sn_stream {\tl_use:N \g__sn_filename_tl .nodes}
    \bool_gset_true:N \g__sn_stream_bool
  }
}

\AtEndDocument
{
  \ExplSyntaxOn
  \bool_if:NT \g__sn_stream_bool
  {
    \iow_close:N \g__sn_stream
  }
  \ExplSyntaxOff
}
\makeatletter
\cs_set_eq:NN \tikz_set_node_name:n \tikz@pp@name
\cs_set_eq:NN \tikz_fig_must_be_named: \tikz@fig@mustbenamed

\cs_new_nopar:Npn \tikz_scan_point:n #1
{
  \tikz@scan@one@point\pgfutil@firstofone#1\relax
}

\cs_new_nopar:Npn \tikz_scan_point:NNn #1#2#3
{
  \tikz@scan@one@point\pgfutil@firstofone#3\relax
  \dim_set_eq:NN #1 \pgf@x
  \dim_set_eq:NN #2 \pgf@y
}

\makeatother
\cs_generate_variant:Nn \tikz_scan_point:n {V}
\cs_generate_variant:Nn \tikz_scan_point:NNn {NNV}
\cs_new_nopar:Npn \save_nodes:Nn #1#2
{
  \tl_clear:N \l__sn_tmpa_tl
  \tikz_scan_point:NNn \l__sn_x_dim \l__sn_y_dim {(current~ bounding~ box.center)}
  \dim_set:Nn \l__sn_x_dim {-\l__sn_x_dim}
  \dim_set:Nn \l__sn_y_dim {-\l__sn_y_dim}
  \tl_set:Nx \l__sn_centre_tl {
    {1}{0}{0}{1}{\dim_use:N \l__sn_x_dim}{\dim_use:N \l__sn_y_dim}
  }
  \clist_map_inline:nn {#2}
  {
    \tl_if_exist:cT {pgf@sh@ns@##1}
    {
      \clist_map_inline:nn {ns,np,ma,pi}
      {
        \tl_put_right:Nn \l__sn_tmpa_tl
        {
          \tl_gset:cn {pgf@sh@####1@ \tikz_set_node_name:n{##1} }
        }
        \tl_if_exist:cTF {pgf@sh@####1@##1}
        {
          \tl_put_right:Nx \l__sn_tmpa_tl {
            {\exp_not:v {pgf@sh@####1@ \tikz_set_node_name:n {##1}}}
          }
        }
        {
          \tl_put_right:Nx \l__sn_tmpa_tl {{}}
        }
      }
      \tl_put_right:Nn \l__sn_tmpa_tl
      {
        \tl_gset:cn {pgf@sh@nt@ \tikz_set_node_name:n{##1} }
      }
      \compose_transformations:NVv \l__sn_tmpb_tl \l__sn_centre_tl {pgf@sh@nt@##1}
      \tl_put_right:Nx \l__sn_tmpa_tl {{\exp_not:V \l__sn_tmpb_tl}}
      \tl_put_right:Nn \l__sn_tmpa_tl {
        \transform_node:Nn \l__sn_transformation_tl {
          \tikz_set_node_name:n{##1}
        }
      }
    }
  }
  \tl_set_eq:NN #1 \l__sn_tmpa_tl
}
\cs_new_nopar:Npn \save_nodes_to_list:nn #1#2
{
  \save_nodes:Nn \l__sn_tmpa_tl {#2}
  \prop_gput:NnV \g__sn_prop {#1} \l__sn_tmpa_tl
}
\cs_new_nopar:Npn \save_nodes_to_file:n #1
{
  \save_nodes:Nn \l__sn_tmpa_tl {#1}
  \sn_open_stream:
  \iow_now:Nx \g__sn_stream
  {
    \iow_newline:
    \exp_not:V \l__sn_tmpa_tl
    \iow_newline:
  }
}
\cs_generate_variant:Nn \save_nodes_to_list:nn {VV}
\cs_generate_variant:Nn \save_nodes_to_file:n {V}
\cs_new_nopar:Npn \restore_nodes_from_list:n #1
{
  \prop_get:NnNT \g__sn_prop {#1} \l__sn_tmpa_tl
  {
    \tl_use:N \l__sn_tmpa_tl
  }
}
\cs_new_nopar:Npn \restore_nodes_from_file:n #1
{
  \file_if_exist:nTF {#1.nodes}
  {
    \msg_log:nnn {tikzmark} {loading nodes} {#1}
    \ExplSyntaxOn
    \file_input:n {#1.nodes}
    \ExplSyntaxOff
  }
  {
    \msg_warning:nnn {tikzmark} {no file} {#1}
  }
}
\AtBeginDocument{\bool_gset_false:N \g__sn_preamble_bool}

\cs_new_nopar:Npn \compose_transformations:Nnn #1#2#3
{
  \tl_gset:Nx #1
  {
    {\fp_eval:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {1}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {2}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {1}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {2}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {3}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {4}
      }
    }
    {\fp_eval:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {3}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {4}
      }
    }
    {\fp_to_dim:n {
        \tl_item:nn {#2} {1}
        * \tl_item:nn {#3} {5}
        +
        \tl_item:nn {#2} {3}
        * \tl_item:nn {#3} {6}
        +
        \tl_item:nn {#2} {5}
      }
    }
    {\fp_to_dim:n {
        \tl_item:nn {#2} {2}
        * \tl_item:nn {#3} {5}
        +
        \tl_item:nn {#2} {4}
        * \tl_item:nn {#3} {6}
        +
        \tl_item:nn {#2} {6}
      }
    }
  }
}
\cs_generate_variant:Nn \compose_transformations:Nnn {cVv,NVv,NVn,NvV,NnV}
\cs_new_nopar:Npn \transform_node:Nn #1#2
{
  \compose_transformations:cVv {pgf@sh@nt@#2} #1 {pgf@sh@nt@#2}
}
\cs_new_nopar:Npn \set_transform_from_node:n #1
{
  \tl_set_eq:Nc \l__sn_transformation_tl {pgf@sh@nt@#1}
  \tikz_scan_point:NNn \l__sn_x_dim \l__sn_y_dim {(#1.center)}

  \dim_set:Nn \l__sn_x_dim {\l__sn_x_dim - \tl_item:cn {pgf@sh@nt@#1}{5}}
  \dim_set:Nn \l__sn_y_dim {\l__sn_y_dim - \tl_item:cn {pgf@sh@nt@#1}{6}}

  \compose_transformations:NnV  \l__sn_transformation_tl {
    {1}{0}{0}{1}{\dim_use:N \l__sn_x_dim}{\dim_use:N \l__sn_y_dim}
  } \l__sn_transformation_tl
}
\cs_generate_variant:Nn \set_transform_from_node:n {v}
\tikzset{
  set~ saved~ nodes~ file~ name/.code={
    \tl_gset:Nx \g__sn_filename_tl {#1}
  },
  transform~ saved~ nodes/.code={
    \set_transform_from_node:v {tikz@last@fig@name}
  },
  set~ node~ group/.code={
    \tl_set:Nn \l__sn_group_tl {#1}
    \pgfkeysalso{
      execute~ at~ end~ scope={
        \maybe_save_nodes:
      }
    }
  },
  save~ nodes~ to~ file/.code={
    \tl_if_eq:nnTF {#1}{false}
    {
      \bool_set_false:N \l__sn_file_bool
    }
    {
      \bool_set_true:N \l__sn_file_bool
    }
    \pgfkeysalso{
      execute~ at~ end~ scope={
        \maybe_save_nodes:
      }
    }
  },
  save~ node/.code={
    \tikz_fig_must_be_named:
    \pgfkeysalso{append~ after~ command={
        \pgfextra{
          \clist_gput_right:Nv \l__sn_nodes_clist {tikz@last@fig@name}
        }
      }
    }
  },
  restore~ nodes~ from~ file/.code={
    \bool_if:NTF \g__sn_preamble_bool
    {
      \restore_nodes_from_file:n {#1}
    }
    {
      \tikz_fig_must_be_named:
      \pgfkeysalso{append~ after~ command={
          \pgfextra{
            \scope
            \split_argument:NNn \tikzset \restore_nodes_from_file:n {#1}
            \endscope
          }
        }
      }
    }
  },
  restore~ nodes~ from~ file/.default = \g__sn_filename_tl,
  restore~ nodes~ from~ list/.code={
    \tikz_fig_must_be_named:
    \pgfkeysalso{append~ after~ command={
        \pgfextra{
          \scope
          \split_argument:NNn \tikzset \restore_nodes_from_list:n {#1}
          \endscope
        }
      }
    }
  }
}
\cs_generate_variant:Nn \clist_gput_right:Nn {Nv}
\cs_new_nopar:Npn \split_argument:NNn #1#2#3
{
  \tl_set:Nx \l__sn_tmpa_tl {\tl_head:n {#3}}
  \tl_if_eq:NNTF \l__sn_tmpa_tl \l__open_bracket_tl
  {
    \split_argument_aux:NNp #1#2#3
  }
  {
    #2 {#3}
  }
}
\cs_new_nopar:Npn \split_argument_aux:NNp #1#2[#3]#4
{
  #1 {#3}
  #2 {#4}
}
\cs_new_nopar:Npn \maybe_save_nodes:
{
  \clist_if_empty:NF \l__sn_nodes_clist
  {
    \bool_if:NTF \l__sn_file_bool
    {
      \save_nodes_to_file:V \l__sn_nodes_clist
    }
    {
      \tl_if_empty:NF \l__sn_group_tl
      {
        \save_nodes_to_list:VV \l__sn_group_tl \l__sn_nodes_clist
      }
    }
    \clist_gclear:N \l__sn_nodes_clist
  }
}
\ExplSyntaxOff
%% 
%% Copyright (C) 2011-2021 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzlibrarytikzmark.code.tex'.


==> tikzmarklibrarylistings.code.tex <==
%%
%% This is file `tikzmarklibrarylistings.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tikzmark.dtx  (with options: `listings')
%% ----------------------------------------------------------------
%% tikzmark --- remembering absolute positioning with TikZ.
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\@ifpackageloaded{listings}{%
  \newif\iflst@linemark
  \lst@linemarktrue
\lst@AddToHook{EveryLine}{%
  \begingroup
  \advance\c@lstnumber by 1\relax
  \pgfmark{line-\lst@name-\the\c@lstnumber-start}%
  \endgroup
}
\lst@AddToHook{EOL}{\pgfmark{line-\lst@name-\the\c@lstnumber-end}%
\global\lst@linemarktrue
}
\lst@AddToHook{OutputBox}{%
  \iflst@linemark
  \pgfmark{line-\lst@name-\the\c@lstnumber-first}%
  \global\lst@linemarkfalse
  \fi
}
\def\tkzmk@lst@fnum#1\relax#2\@STOP{%
  \def\@test{#2}%
  \ifx\@test\@empty
  \def\tkzmk@lst@start{0}%
  \else
  \@tempcnta=#1\relax
  \advance\@tempcnta by -1\relax
  \def\tkzmk@lst@start{\the\@tempcnta}%
  \fi
}
\lst@AddToHook{Init}{%
  \expandafter\tkzmk@lst@fnum\lst@firstnumber\relax\@STOP
  \pgfmark{line-\lst@name-\tkzmk@lst@start-start}%
}
}{%
    \PackageError{tikzmark listings}{The listings package has not been loaded.}{}
}
%% 
%% Copyright (C) 2011-2021 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the file  tikzmark.dtx
%% and the derived files           tikzmark.ins,
%%                                 tikzmark.pdf,
%%                                 tikzlibrarytikzmark.code.tex, and
%%                                 tikzmarklibrarylistings.code.tex
%% 
%%
%% End of file `tikzmarklibrarylistings.code.tex'.

